Totally geodesic surfaces in twist knot complements

In this article, we give explicit examples of infinitely many non-commensurable (non-arithmetic) hyperbolic $3$-manifolds admitting exactly $k$ totally geodesic surfaces for any positive integer $k$, answering a question of Bader, Fisher, Miller and Stover. The construction comes from a family of twist knot complements and their dihedral covers. The case $k=1$ arises from the uniqueness of an immersed totally geodesic thrice-punctured sphere, answering a question of Reid. Applying the proof techniques of the main result, we explicitly construct non-elementary maximal Fuchsian subgroups of infinite covolume within twist knot groups, and we also show that no twist knot complement with odd prime half twists is right-angled in the sense of Champanerkar, Kofman, and Purcell.

==> ThriceVert.tex <==

\begin{tikzpicture}[thick]
\def\rim{0.07}
% % Pic
\begin{scope}
% \clip [name path global=clip] (-0.25,-3) rectangle (4.25,3); % small
\clip [name path global=clip] (-0.25,-3) rectangle (6.25,3); % big
% % punctures
\foreach \i in {0,1,2,3}
  {
  \draw [\acol,name path global=1v\i] (4*\i,-3) -- ++ (0,6);     % 1st
  \draw [\bcol,name path global=2v\i] (4*\i+2,-3) -- ++ (0,6);   % 2nd
  }
% % Long puncture
\foreach \i in {0,1,2,3}
  {\draw [\lcol,name path global=slant\i] (-1,4*\i) -- ++ (8,-16);}
\end{scope}
% % Slant intersections
\path [name intersections={of=1v0 and slant0,by=origin}];
  \fill (origin) circle (\rim) node [left] {$0$};
\path [name intersections={of=1v0 and slant1,by=upper}];
  \fill (upper) circle (\rim) node [left] {$1$};
\path [name intersections={of=2v0 and slant1,by=tau}];
  \fill (tau) circle (\rim) node [above right] {$1-\tau$};
% % Vertical intersections
%\foreach \i in {0,1,2,3}
%  {
%    \path [name intersections={of=clip and 1v\i,by={1a\i,1b\i}}];
%    \path [name intersections={of=clip and 2v\i,by={2a\i,2b\i}}];
%  }
\path [name intersections={of=clip and 1v0,by={1a0,1b0}}]
  \node [\acol,above] at (1a0) {$\BH_{\BR}2$};
\path [name intersections={of=clip and slant1,by={UL,DR}}];
  \node [\lcol,above left] at (UL) {$w_j^{-1}(\BH_{\BR}^2)$};
% % Fundom
\begin{scope}[on background layer]
\path [name path global=fundom] (origin) rectangle ++ (4,4);
\fill [use path=fundom,\bcol!10];
\end{scope}
\draw [use path=fundom,dashed,line width=0.5mm];
\end{tikzpicture}

==> ThriceVertRight.tex <==

\begin{tikzpicture}[thick]
\def\rim{0.07}
% % Pic
\begin{scope}
\clip [name path global=clip] (-0.25,-3) rectangle (4.25,3);
% % punctures
\foreach \i in {0,1,2,3}
  {
  \draw [\acol,name path global=1v\i] (4*\i,-3) -- ++ (0,6);     % 1st
  \draw [\bcol,name path global=2v\i] (4*\i+2,-3) -- ++ (0,6);   % 2nd
  }
% % Long puncture
\foreach \i in {0,1,2,3,4,5,6,7}
  {\draw [\lcol,name path global=slant\i] (-1,4*\i) -- ++ (8,-16);}
\end{scope}
% % Slant intersections
% \path [name intersections={of=1v0 and slant0,by=origin}];
%   \fill (origin) circle (\rim) node [left] {$0$};
\path [name intersections={of=1v0 and slant1,by=upper}];
  \fill (upper) circle (\rim) node [left] {$0$};
\path [name intersections={of=2v0 and slant1,by=tau}];
  \fill (tau) circle (\rim) node [above right] {$2-\tau$};
% % Vertical intersections
\foreach \i in {0,1,2,3}
  {
    \path [name intersections={of=clip and 1v\i,by={1a\i,1b\i}}];
    \path [name intersections={of=clip and 2v\i,by={2a\i,2b\i}}];
  }
  \node [\acol,above] at (1a0) {$\BH_{\BR}^2$};
\path [name intersections={of=clip and slant1,by={UL,DR}}];
  \node [\lcol,above left] at (UL) {$w_j^{-1}(\BH_{\BR}^2)$};
% % Angles
\begin{scope}[on background layer]
\clip (1a0) -- (upper) -- (tau) -- (2a0) -- cycle;
\draw (upper) circle (5*\rim);
\end{scope}
\end{tikzpicture}

==> ThriceVertSurf.tex <==

\begin{tikzpicture}[thick]
\def\rim{0.07}
% % Pic
\begin{scope}
\clip [name path global=clip] (-0.25,-3) rectangle (4.25,3); % small
% \clip [name path global=clip] (-0.25,-3) rectangle (6.25,3); % big
% % punctures
\foreach \i in {0,1,2,3}
  {
  \draw [\acol,name path global=1v\i] (4*\i,-3) -- ++ (0,6);     % 1st
  \draw [\bcol,name path global=2v\i] (4*\i+2,-3) -- ++ (0,6);   % 2nd
  }
% % Long puncture
\foreach \i in {0,1,2,3}
  {\draw [\lcol,name path global=slant\i] (-1,4*\i) -- ++ (8,-16);}
\end{scope}
% % Slant intersections
\path [name intersections={of=1v0 and slant0,by=origin}];
  \fill (origin) circle (\rim) node [left] {$0$};
\path [name intersections={of=1v0 and slant1,by=upper}];
  \fill (upper) circle (\rim) node [left] {$1$};
\path [name intersections={of=2v0 and slant1,by=tau}];
  \fill (tau) circle (\rim) node [above right] {$1-\tau$};
% % Vertical intersections
%\foreach \i in {0,1,2,3}
%  {
%    \path [name intersections={of=clip and 1v\i,by={1a\i,1b\i}}];
%    \path [name intersections={of=clip and 2v\i,by={2a\i,2b\i}}];
%  }
\path [name intersections={of=clip and 1v0,by={1a0,1b0}}]
  \node [\acol,above] at (1a0) {$\BH_{\BR}2$};
\path [name intersections={of=clip and slant1,by={UL,DR}}];
  \node [\lcol,above left] at (UL) {$w_j^{-1}(\BH_{\BR}^2)$};
% % Sigma surface
\begin{scope}
\clip [use path=clip];
\draw [\sigcol,name path global=sig] (-1,4*0.6) -- ++ (8,-16);
\end{scope}
\path [name intersections={of=clip and sig,by={ul,dr}}];
  \node [\sigcol,above left] at (ul) {$\widetilde{\Sigma}$};
\path [name intersections={of=1v0 and sig,by=mid}];
  \fill (mid) circle (\rim) node [left] {$s/t$};
\end{tikzpicture}
